Rephotography in the Digital Era: Mass Rephotography and re.photos, the Web Portal for Rephotography

Since the beginning of rephotography in the middle of the 19th century, techniques in registration, conservation, presentation, and sharing of rephotographs have come a long way. Here, we will present existing digital approaches to rephotography and discuss future approaches and requirements for digital mass rephotography. We present re.photos, an existing web portal for rephotography, featuring methods for collaborative rephotography, interactive image registration, as well as retrieval, organization, and sharing of rephotographs. For mass rephotography additional requirements must be met. Batches of template images and rephotographs must be handled simultaneously, image registration must be automated, and intuitive smartphone apps for rephotography must be available. Long--term storage with persistent identifiers, automatic or mass georeferencing, as well as gamification and social media integration are further requirements we will discuss in this paper.

==> acronyms.tex <==
% Acronyms %%%%%%%%%%%%%%%%%%%%%%%%%%%%
%ac normal
%acf full if later ac is called full again
%acl long without mentioning acronym
\newacronym{aaap}{aaap}{as affine as possible}

\newacronym{acm}{ACM}{Association for Computing Machinery}

\newacronym{acr}{ACR}{active camera relocalization}

\newacronym{ai}{AI}{artificial intelligence}

\newacronym{ann}{ANN}{artificial neural network}

\newacronym{aoi}{AOI}{area of interest}

\newacronym{ar}{AR}{Augmented reality}

\newacronym{cnn}{CNN}{convolutional neural network}

\newacronym{dem}{DEM}{Digital Elevation Model}

\newacronym{dof}{DOF}{depth of field}

\newacronym{dorelu}{doReLU}{Double Rectified Linear Unit}

\newacronym{dslr}{DSLR camera}{digital single lens reflex camera}

\newacronym{eg}{EG}{Eurographics}

\newacronym{fff}{FFF}{Fused Filament Fabrication}

\newacronym{fsa}{FSA}{Farm Security Administration}

\newacronym{gan}{GAN}{generative adversarial network}

\newacronym{gbl}{GBL}{Game Based Learning}

\newacronym{gcp}{GCP}{ground control point}

\newacronym{gif}{GIF}{Graphics Interchange Format}

\newacronym{gis}{GIS}{geographic information system}

\newacronym{gpl}{GPL}{GNU General Public License}

\newacronym{gps}{GPS}{Global Positioning System}

\newacronym{hci}{HCI}{human-computer interaction}

\newacronym{hdri}{HDRI}{high-dynamic-range imaging}

\newacronym{hsi}{HSI}{habitat suitability model}

\newacronym{ieee}{IEEE}{Institute of Electrical and Electronics Engineers}

\newacronym{insticc}{INSTICC}{Institute for Systems and Technologies of Information, Control and Communication}

\newacronym{js}{JS}{JavaScript}

\newacronym{ki}{KI}{Künstliche Intelligenz}

\newglossaryentry{knn}
{
  name={KNN},
  description={Künstliches Neuronales Netz},
  first={\glsentrydesc{knn} (\glsentrytext{knn})},
  plural={KNNs},
  firstplural={Künstliche Neuronale Netze (\glsentryplural{knn})}
}

%\newacronym{}{KNN}{Künstliches Neuronales Netz}

\newacronym{lia}{LIA}{Little Ice Age}

\newacronym{lidar}{LIDAR}{light detection and ranging}

\newacronym{mdia}{MDIA}{multi-data integrative analysis}

\newacronym{mlp}{MLP}{multilayer perceptron}

\newacronym{mnn}{MNN}{Mechanical Neural Network}

\newacronym{mnnde}{MNN}{Mechanisches Neuronales Netz}

\newacronym{nasa}{NASA}{National Aeronautics and Space Administration}

\newacronym{ngs}{NGS}{U.S. National Geodetic Survey}

\newacronym{ppm}{PPM}{photopointmonitoring}

\newacronym{relu}{ReLU}{Rectified Linear Unit}

\newacronym{sift}{SIFT}{scale-invariant feature transform}

\newacronym{siggraph}{SIGGRAPH}{Special Interest Group on Computer Graphics and Interactive Techniques}

\newacronym{sits}{SITS}{Satellite Image Time Series}

\newacronym{sla}{SLA}{Stereolithografie}

\newacronym{swk}{SWK}{Ständige Wissenschaftliche Kommission der Kultusministerkonferenz}

\newacronym{uav}{UAV}{unmanned aerial vehicle}

\newacronym{usgs}{USGS}{United States Geological Survey}

\newacronym{vr}{VR}{Virtual reality}

\newacronym{vrp}{VRP}{virtual repeat photography}

\newacronym{wave}{WAVE}{Wide-Area Visualisation environment}

\newacronym{wscg}{WSCG}{World Society for Computer Graphics}

\newacronym{wwi}{WWI}{World War I}

\newacronym{wwii}{WWI}{World War II}

\newacronym{fcd}{FCD}{Floating Car Data}
\newacronym{vmz}{VMZ}{Verkehrsmanagementzentrale}
\newacronym{vmznds}{VMZNDS}{Verkehrsmanagementzentrale Niedersachsen}
\newacronym{nlstbv}{NLStBV}{Niedersächsische Landesbehörde für Straßenbau und Verkehr}
\newacronym{vnrw}{VNRW}{Verkehr.NRW}
\newacronym{snrw}{Straßen.NRW}{Landesbetrieb Straßenbau Nordrhein-Westfalen}
\newacronym{los}{LOS}{Level of Service}
\newacronym{wms}{WMS}{Web Map Service}
\newacronym{bkg}{BKG}{Bundesamt für Kartographie und Geodäsie}
\newacronym{teu}{TEU}{Traffic Eye Universal}
\newacronym{lstm}{LSTM}{Long Short Term Memory}
\newacronym{gru}{GRU}{Gated Recurrent Units}
\newacronym{nn}{NN}{Neural Network}
\newacronym{gnn}{GNN}{Graph Neural Network}
\newacronym{udp}{UDP}{Urban Data Plattform}
\newacronym{oup}{OUP}{Open Urban Plattform}
\newacronym{uvm}{UVM}{Umweltsensitives Verkehrsmanagement}
\newacronym{usp}{USP}{Unique Selling Proposition}
\newacronym{hbefa}{HBEFA}{Handbuch für Emissionsfaktoren des Straßenverkehrs}
\newacronym{anpr}{ANPR}{Automatic number-plate recognition}
\newacronym[plural={Lichtsignalanlagen}, firstplural=Lichtsignalanlagen (LSAs)]{lsa}{LSA}{Lichtsignalanlage}
\newacronym{öpnv}{ÖPNV}{Öffentliche Personennahverkehr}
\newacronym{dsgvo}{DSGVO}{Datenschutz-Grundverordnung}
\newacronym{thg}{THG}{Treibhausgas-Emission}
\newacronym{osm}{OSM}{OpenStreetMap}
\newacronym{agb}{AGB}{Allgemeine Geschäftsbedingungen}
\newacronym{fgsv}{FGSV}{Forschungsgesellschaft für Straßen- und Verkehrswesen}
\newacronym{maas}{MaaS}{Mobility as a Service}
\newacronym{llm}{LLM}{large language model}

